Crossing the Cyber Divide: Sim-to-Sim and Sim-to-Real Transfer for RL Agents

Cyber attack agents are typically trained and evaluated within a single simulator, making it unclear whether learned policies transfer beyond the environments in which they were developed. This limitation hinders both deployment and fair comparison, as cyber simulators differ substantially in their state representations, observation models, and action spaces. In this paper, we study policy transfer across cyber environments and argue that simulator-to-simulator and simulator-to-real transfer can be viewed as instances of the same underlying alignment problem. We propose a framework that separates state alignment from action translation, enabling a policy trained in one environment to operate in another without retraining. We evaluate transfer across four cyber platforms, CyberBattleSim, NetSecGame, CyberWheel, and NASim, including emulated deployments in NASim. Our experiments show that zero-shot transfer is feasible, fully preserving source-policy performance in closely aligned environments and achieving 45.2% win rates when transferring policies whose source performance is 60.5%. In emulated virtual machine environments, transferred policies exhibit a Jensen-Shannon divergence of 0.085 from native policies, indicating strong behavioral similarity. Code and benchmarks are available at: https://anonymous.4open.science/r/RL-Transfer-between-env-4F47/.

==> Sections/5_transfer._old.tex <==

\section{Transfer Components}
\label{sec:method}
 
\begin{figure}[t]
\centering
\framebox[\textwidth]{\rule{0pt}{6cm}}
\caption{Placeholder for diagram.}
\label{fig:diagram}
\end{figure}

 
\subsection{Action Transfer: Kill-Chain Translation Layer}
\label{sec:kc}
 
The CW~policy produces a discrete slot in $\{0,\ldots,12\}$.
\CBS requires a structured (source\_node, target\_node, vulnerability\_id) triple or a local\_vulnerability(node, vuln\_id) call.
The kill-chain translation layer (v1) bridges these by maintaining a per-slot phase counter \texttt{\_slot\_cw\_phases} and translating as follows:
 
\begin{itemize}
  \item \textbf{Phases~0--2} (\texttt{ping\_sweep}, \texttt{port\_scan}, \texttt{svc\_disc}): Issue \texttt{local\_vulnerability} on the current frontier owned node, cycling through \CBS vulnerability indices.
  \item \textbf{Phase~3} (\texttt{exploit}): Attempt \texttt{connect(src $\to$ target)} if a relevant credential is present in the \CBS cache; otherwise retry \texttt{local\_vulnerability}.
  \item \textbf{Phase~4+}: Issue \texttt{local\_vulnerability} on the current owned node, cycling through all available vulnerabilities.
\end{itemize}
 
Two design properties are critical for interpreting results.
First, the kill-chain phase labels are cosmetic---the layer does not perform actual network reconnaissance.
During phases~0--2, it executes local vulnerability exploitation regardless of the label.
Second, during phases~0--2, the policy's slot choice has \emph{no effect} on the \CBS action taken: all slots produce the same \texttt{local\_vulnerability} call.
The CW~policy's learned preferences only become operationally relevant during phase~3 and beyond, when credential-based lateral movement introduces a genuine choice of target.
This structural property directly explains the main empirical finding (\cref{sec:analysis}).
 
\subsection{State Transfer: Domain-Adversarial Prototypical Network}
\label{sec:dapn}
 
The CW~policy expects a 512-dimensional observation encoding kill-chain state across up to 100~hosts.
Presenting raw \CBS observations---also 512~dimensions after preprocessing, but with entirely different internal structure---results in distributional mismatch severe enough to cause the policy to produce only no-op actions (0\% win rate, 0.00~mean nodes owned; see \cref{sec:results}).
 
The \DAPN encoder maps \CBS observations into the 512-dimensional representation expected by the CW~policy using three alignment objectives:
%
\begin{enumerate}
  \item A DAPN-style domain adversarial loss~\cite{ganin2015dann} that encourages encoder outputs to be indistinguishable between CW and \CBS domains.
  \item A stage prediction loss that aligns encoded representations by kill-chain progression stage.
  \item A pair alignment loss that minimises the distance between CW and \CBS encodings collected under semantically equivalent attack states.
\end{enumerate}
 
Training uses 2{,}000 paired CW/\CBS observations collected by running the CW~policy in \CW and a scripted agent in \CBS across comparable attack scenarios.
Phase values in $[0.0, 1.0]$ are injected into the \CBS \texttt{nodes\_privilegelevel} component before encoding.
The encoder is trained for 50~epochs on CPU.
 
The \DAPN encoder is integrated with the translation layer via the KCDAPNTranslateWrapper, which applies the encoder to each \CBS observation before returning it to the policy.



==> Sections/5_transfer.tex <==
\section{Transfer Components}
\label{sec:method}
 


\subsection{Action Transfer: Kill-Chain Translation Layer}
\label{sec:kc}

The kill-chain translation layer implements $\psi: \mathcal{A}_A \rightarrow
\mathcal{A}_B$ by maintaining a per-slot phase counter and mapping each slot
to the appropriate target-native action. For the CW$\rightarrow$\CBS
transfer, the CW policy produces a slot in $\{0,\ldots,12\}$ which is
translated to a (source, target, vulnerability) triple required by \CBS.

The mapping proceeds by kill-chain phase:

\begin{itemize}[leftmargin=*,
    topsep=0pt,
    partopsep=0pt,
    parsep=0pt,
    itemsep=0pt]
  \item \noindent \textbf{Phases 0--2} (reconnaissance): Issue a local exploitation
  call on the current frontier node, cycling through available vulnerability
  indices.
  \item \noindent \textbf{Phase 3} (exploit): Attempt lateral movement if a credential
  is cached; otherwise retry local exploitation.
  \item \noindent \textbf{Phase 4+}: Issue local exploitation on the current owned
  node, cycling all available vulnerabilities.
\end{itemize}

Two properties bear directly on the results. (1) During phases 0--2 all
slots produce the same call, so $\psi$ is effectively constant and the
policy's learned preferences have no operational effect until phase 3, when
lateral movement introduces a genuine target choice. (2) No actual
network reconnaissance is performed; $\psi$ only sequences exploitation
calls.

\subsection{State Transfer: DAPN Data Collection and Training}
\label{sec:dapn}

The \DAPN encoder implements $E_\theta: \phi(\mathcal{S}_B) \rightarrow
\mathcal{S}_A$, closing the distributional gap that remains after $\phi$ is
applied. For the CW$\rightarrow$\CBS transfer, the encoder maps
512-dimensional \CBS observations into the representation expected by the CW
policy, trained on 2{,}000 paired observations. For other environments, see the dimension specifications in Table \ref{tab:envs}. At inference, the wrapper
composes $\phi$, $E_\theta$, and $\psi$ into a single pipeline delivering
$\psi(E_\theta(\phi(s_B)))$ to $\mathcal{M}_B$ keeping
$\pi_A$ unchanged.

==> Sections/7_discussion.tex <==
\section{Discussion}
\label{sec:discussion}
 
\subsection{Failure Modes and Limits}
 
The No~DAPN condition reveals a critical failure mode: naive observation preprocessing - dimensionality alignment without distributional alignment---is entirely insufficient.
The CW~policy does not merely underperform on raw \CBS observations; it produces essentially random no-op output.
This failure is total, not graceful.
 
Several additional limitations bound the generalisability of current results: the chain topology provides minimal decision branching; the \DAPN encoder is trained on only 2{,}000 paired observations; the translation layer~(v1) is open-loop and does not adapt to observation feedback; and injected phase values are synthetic approximations rather than direct observations.
Each limitation is a concrete engineering problem with a clear path to improvement (\cref{sec:future}).
 
\subsection{Implications for Deployed Red-Team Tooling}
 
For linear, sequential attack paths---which characterise many penetration testing workflows, including initial access followed by staged lateral movement through a fixed credential chain---the kill-chain translation layer alone is sufficient, and retraining policies for each target environment is unnecessary.
For branching attack graphs where the agent must choose among multiple viable paths, state encoder guidance becomes more critical, and higher-quality alignment is likely required.
 
The cost comparison is favourable: \DAPN requires 2{,}000 paired observations and 50~training epochs---modest relative to 200{,}000~timesteps of policy training from scratch.
If the encoder provides meaningful benefits on harder topologies, this represents a favourable cost/benefit tradeoff for deployment workflows.
 
A practical implication for tooling design: win rate is a poor metric for evaluating state encoders when the action translation layer is itself sufficient for task completion.
Metrics that measure step efficiency, progress rate, or performance on harder instances (more nodes required, tighter budgets, branching topologies) are needed to distinguish the contributions of the two transfer components.
 
The \NSG results sharpen this picture.
When a target environment natively shares the source environment's observation schema---as \NSG shares \CW's kill-chain feature format---direct deployment is viable and achieves non-trivial win rates without any representational bridge.
Operators working across environments that share common feature vocabularies (e.g., two kill-chain-based simulators, or a simulator and an emulation environment with structured kill-chain instrumentation) may not need an encoder at all.
The \DAPN encoder then functions as a refinement step, correcting for distributional differences at the transition-dynamic level that are invisible in the feature schema but present in the collected observation statistics.
 

==> Sections/8_future_work.tex <==
\section{Future Work}
